Symbolic Brittleness in Sequence Models: on Systematic Generalization in Symbolic Mathematics

Neural sequence models trained with maximum likelihood estimation have led to breakthroughs in many tasks, where success is defined by the gap between training and test performance. However, their ability to achieve stronger forms of generalization remains unclear. We consider the problem of symbolic mathematical integration, as it requires generalizing systematically beyond the test set. We develop a methodology for evaluating generalization that takes advantage of the problem domain's structure and access to a verifier. Despite promising in-distribution performance of sequence-to-sequence models in this domain, we demonstrate challenges in achieving robustness, compositionality, and out-of-distribution generalization, through both carefully constructed manual test suites and a genetic algorithm that automatically finds large collections of failures in a controllable manner. Our investigation highlights the difficulty of generalizing well with the predominant modeling and learning approach, and the importance of evaluating beyond the test set, across different aspects of generalization.

==> figures/fitness_distribution.tex <==
\begin{figure}
\begin{center}
\footnotesize
\includegraphics[width=0.8\linewidth]{images/node_dist_general.png}
\caption{\label{fig:node_dist_general} Node distribution for a 1,000 problem archive of general failures from SAGGA using diversity or high-fitness seed selection. Diverse seed selection yields a more diverse node distribution.
}
\end{center}
\end{figure}

==> figures/method_figure.tex <==
\begin{figure*}
\begin{center}
\footnotesize
\includegraphics[width=0.99\linewidth]{images/method_fig.pdf}
\caption{\label{fig:fig1} Methods employed here to probe aspects of systematic generalization: \textit{manual perturbation} to test robustness, \textit{example combination} to test compositionality, and \textit{automatic example evolution} (the SAGGA algorithm) to discover adversarial failure cases.
}
\end{center}
\end{figure*}

==> tables/genetic.tex <==
%
\begin{table}[t!]
\setlength{\tabcolsep}{6pt}
\footnotesize
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Type} & \textbf{Cluster 1} & \textbf{Cluster 2} & \textbf{Cluster 3} & \textbf{Cluster 4} & \textbf{Cluster 5}\\
\midrule
\texttt{robustness} & $-590$ & $214$ & $x^{311} + 10$ & $277 + x^{-71}$ & $128 + x^{-970}$ \\
& $-670$ & $233$ & $x^{311} + 133$ & $336 + x^{-71}$ & $171 + x^{-261}$ \\
& $-690$ & $293$ & $x^{311} + 139$ & $693 + x^{-71}$ & $176 + x^{-261}$ \\
\midrule
\texttt{general}& $-182$ & $107^x$ & $2/x^3$ & $-128*x^{x + 2}$ & $0^{x^2} + x^2 + 7/x^3$ \\
& $-241$ & $123^x$ & $4/x^3$ & $-349*x^{x + 2}$ & $2^{3/x^{190}} + 1$ \\
& $-469$ & $167^x$ & $7/x^3$ & $-386*x^{x + 1}$ & $2^{x^{259*x}} + x^4 + 37$ \\
\bottomrule
\end{tabular}
}
\caption{\label{tbl:prediction-examples} 
The neural sequence integrator fails to integrate each of these problems discovered by SAGGA.
\textbf{Top:} SAGGA reveals failures related to integer mutations, including negative (Cluster 1) or positive (Cluster 2) integers, or exponents (Clusters 3-5).
\textbf{Bottom:} SAGGA discovers  integer (Cluster 1), exponent (Cluster 3), and more complex (Cluster 5) failures. 
}
\end{center}
\end{table}
%
